Gradient Imitation Reinforcement Learning for General Low-Resource Information Extraction

Information Extraction (IE) aims to extract structured information from heterogeneous sources. IE from natural language texts include sub-tasks such as Named Entity Recognition (NER), Relation Extraction (RE), and Event Extraction (EE). Most IE systems require comprehensive understandings of sentence structure, implied semantics, and domain knowledge to perform well; thus, IE tasks always need adequate external resources and annotations. However, it takes time and effort to obtain more human annotations. Low-Resource Information Extraction (LRIE) strives to use unsupervised data, reducing the required resources and human annotation. In practice, existing systems either utilize self-training schemes to generate pseudo labels that will cause the gradual drift problem, or leverage consistency regularization methods which inevitably possess confirmation bias. To alleviate confirmation bias due to the lack of feedback loops in existing LRIE learning paradigms, we develop a Gradient Imitation Reinforcement Learning (GIRL) method to encourage pseudo-labeled data to imitate the gradient descent direction on labeled data, which can force pseudo-labeled data to achieve better optimization capabilities similar to labeled data. Based on how well the pseudo-labeled data imitates the instructive gradient descent direction obtained from labeled data, we design a reward to quantify the imitation process and bootstrap the optimization capability of pseudo-labeled data through trial and error. In addition to learning paradigms, GIRL is not limited to specific sub-tasks, and we leverage GIRL to solve all IE sub-tasks (named entity recognition, relation extraction, and event extraction) in low-resource settings (semi-supervised IE and few-shot IE).

==> tables/CDA.tex <==
\begin{table}[bt!]
\centering
% \resizebox{0.95\linewidth}{!}{
\caption{F1 (\%) of {\modelname} with various percentages of labeled data under different LRE scenarios.}\label{tab:CDA_aug}
\begin{tabular}{lcccc}
\thickhline
&\textbf{\% Labeled Data} & \textbf{\textsf{L}} & \textbf{\textsf{L + CDA}} & \textbf{\textsf{L + U}} \\\hline
\multicolumn{1}{c}{\multirow{3}{*}{\textbf{SemEval}}} & 5\%  & 72.71                        & 75.52                     & 79.65                   \\
\multicolumn{1}{c}{}                  & 10\% & 73.93                       & 81.47                    & 81.69                   \\
\multicolumn{1}{c}{}                         & 30\% & 80.55                       & 84.63                    & {85.52}                   \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{\textbf{TACRED}}}  & 3\%  & 41.11                       & 43.34                     & {47.37}                   \\
\multicolumn{1}{c}{}                         & 10\% & 53.23                         & 57.07                     & {58.20}                    \\
\multicolumn{1}{c}{}                         & 15\% & 55.35                        & 58.89                    & {59.93}  \\\thickhline                
\end{tabular}

% \vspace{-0.1in}
\end{table}

==> tables/case_CDA.tex <==
\begin{table}[t!]
\centering
% \resizebox{0.85\linewidth}{!}{
\caption{CDA on labeled data to obtain generated data, where {\color{red}\textit{red}} and {\color{blue}\textit{blue}} represent head and
tail entities respectively, {\color{cyan}\textit{cyan}} represents the replaced words.}\label{tab:CDA_case_study}
\begin{tabular}{l}
\thickhline
\begin{tabular}[c]{@{}l@{}}Original: A {\color{red}\textit{letter}} was {\color{cyan}\textit{delivered to}} my {\color{blue}\textit{office}} in ...
\\ 
{\color{purple}Label}: \textbf{\texttt{Entity-Destination}}\\
Generated: A {\color{red}\textit{letter}} was {\color{cyan}\textit{sent from}} my {\color{blue}\textit{office}} in ...
\\{\color{purple}Pseudo label}: \textbf{\texttt{Entity-Origin}}\end{tabular}     \\
\\
\begin{tabular}[c]{@{}l@{}}Original: The {\color{red}\textit{editor}} improved the {\color{blue}\textit{manuscript}}\\ ${\quad\quad\quad\quad}$ with {\color{cyan}\textit{his changes}}.
\\ 
{\color{purple}Label}: \textbf{\texttt{Product-Producer}}\\
Generated: The {\color{red}\textit{editor}} improved the {\color{blue}\textit{manuscript}}\\ ${\quad\quad\quad\quad}$ with {\color{cyan}\textit{some improvements}}.
\\ {\color{purple}Pseudo label}: \textbf{\texttt{Product-Producer}}\end{tabular} 
\\
\\
\begin{tabular}[c]{@{}l@{}}Original: The  {\color{cyan}\textit{suspect dumped}} the {\color{cyan}\textit{dead}} {\color{red}\textit{body}}\\ ${\quad\quad\quad\quad}$  into a local {\color{blue}\textit{reservoir}}.
\\ 
{\color{purple}Label}: \textbf{\texttt{Entity-Destination}}\\
Generated: The  {\color{cyan}\textit{dam bulids}} the {\color{cyan}\textit{human}} {\color{red}\textit{body}}\\ ${\quad\quad\quad\quad}$  into a local {\color{blue}\textit{reservoir}}.
\\ {\color{purple}Pseudo label}: \textbf{\texttt{Other}}\end{tabular} \\
\thickhline
\end{tabular}

\end{table}

==> tables/case_GIRL_ee_1.tex <==
\begin{table}[t!]
\centering
% \resizebox{0.85\linewidth}{!}{
\caption{Trigger Identification and Classification in Event Extraction with/without {\modelname} on ACE05-E, where {\color{blue}\textit{blue}} represents the Trigger.}
\label{tab:pseudo_label_case_study_ee_1}
\begin{tabular}{l}
\thickhline
\begin{tabular}[c]{@{}l@{}}The president of the United States coming for a brief two-day\\ {\color{blue}\textit{summit}} with the British prime minister Tony Blair.\\ {\color{purple}Label}: \textbf{\texttt{Contact:Meet}}\\{\color{purple}Prediction w/o GIRL}: \textbf{\texttt{No Identification}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{Contact:Meet}}\end{tabular}                                                                 \\
\\
\begin{tabular}[c]{@{}l@{}}The only people who profit from class {\color{blue}\textit{actions}} are the lawyers.\\ {\color{purple}Label}: \textbf{\texttt{Justice:Sue}}\\{\color{purple}Prediction w/o GIRL}: \textbf{\texttt{Justice:Appeal}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{Justice:Sue}}\end{tabular} \\
\\
\begin{tabular}[c]{@{}l@{}}U.S. troops thwarted a Baghdad bank robbery over the {\color{blue}\textit{protests}}\\ of Iraqis eager to share in the loot.\\ {\color{purple}Label}: \textbf{\texttt{Conflict:Demonstrate}}\\ {\color{purple}Prediction w/o GIRL}: \textbf{\texttt{No Identification}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{No Identification}}\end{tabular}                                       \\ \thickhline
\end{tabular}
% \vspace{-0.1in}
\end{table}

==> tables/case_GIRL_ee_2.tex <==
\begin{table}[t!]
\centering
% \resizebox{0.85\linewidth}{!}{
\caption{Argument Identification and Classification in Event Extraction with/without {\modelname} on ACE05-E, where {\color{blue}\textit{blue}} and {\color{red}\textit{red}} represent the Trigger and Argument respectively.}
\label{tab:pseudo_label_case_study_ee_2}
\begin{tabular}{l}
\thickhline
\begin{tabular}[c]{@{}l@{}}Reports suggesting airport {\color{red}\textit{buildings}} have been {\color{blue}\textit{attacked}}, but\\ runways remain operational.\\
{\color{purple}Label}: \textbf{\texttt{Target-Arg}}\\{\color{purple}Prediction w/o GIRL}: \textbf{\texttt{No Identification}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{Target-Arg}}\end{tabular}                                                                 \\
\\
\begin{tabular}[c]{@{}l@{}}At that point the baby's {\color{red}\textit{mother}} {\color{blue}\textit{stabbed}} him right in the hand.\\ {\color{purple}Label}: \textbf{\texttt{Agent-Arg}}\\{\color{purple}Prediction w/o GIRL}: \textbf{\texttt{Victim-Arg}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{Agent-Arg}}\end{tabular} \\
\\
\begin{tabular}[c]{@{}l@{}}If you were president, which national {\color{red}\textit{figures}} would you\\ {\color{blue}\textit{appoint}} to your cabinet and why?\\ {\color{purple}Label}: \textbf{\texttt{Person-Arg}}\\ {\color{purple}Prediction w/o GIRL}: \textbf{\texttt{No Identification}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{No Identification}}\end{tabular}                                       \\ \thickhline
\end{tabular}
% \vspace{-0.1in}
\end{table}

==> tables/case_GIRL_ner.tex <==
\begin{table}[t!]
\centering
% \resizebox{0.85\linewidth}{!}{
\caption{Named Entity Recognition with/without {\modelname} on OntoNotes 5.0, where {\color{blue}\textit{blue}} represents the predicted named entity.}
\label{tab:pseudo_label_case_study_ner}
\begin{tabular}{l}
\thickhline
\begin{tabular}[c]{@{}l@{}}{\color{blue}\textit{Jiujiang}} is the thoroughfare connecting Yangtze River's north...\\ {\color{purple}Label}: \textbf{\texttt{B-GPE}}\\{\color{purple}Prediction w/o GIRL}: \textbf{\texttt{O}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{B-GPE}}\end{tabular}                                                                 \\
\\
\begin{tabular}[c]{@{}l@{}}Tanks currently are defined as armored vehicles weighing {\color{blue}\textit{25 tons}}\\ or more that carry large guns.\\ {\color{purple}Label}: \textbf{\texttt{B-QUANTITY, I-QUANTITY}}\\{\color{purple}Prediction w/o GIRL}: \textbf{\texttt{B-CARDINAL, O}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{B-QUANTITY, I-QUANTITY}}\end{tabular} \\
\\
\begin{tabular}[c]{@{}l@{}}Defense lawyers have said all along that it was Palestinians and\\ not their Libyan clients who bombed {\color{blue}\textit{Pan Am 103}}.\\ {\color{purple}Label}: \textbf{\texttt{B-PRODUCT, I-PRODUCT, I-PRODUCT}}\\ {\color{purple}Prediction w/o GIRL}: \textbf{\texttt{O, O, O}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{B-FAC, I-FAC, I-FAC}}\end{tabular}                                       \\ \thickhline
\end{tabular}
% \vspace{-0.1in}
\end{table}

==> tables/case_GIRL_re.tex <==
\begin{table}[t!]
\centering
% \resizebox{0.85\linewidth}{!}{
\caption{Relation Extraction with/without {\modelname} on SemEval, where {\color{red}\textit{red}} and {\color{blue}\textit{blue}} represent head and
tail entities respectively.}
\label{tab:pseudo_label_case_study_re}
\begin{tabular}{l}
\thickhline
\begin{tabular}[c]{@{}l@{}}My {\color{red}\textit{brother}} has entered my {\color{blue}\textit{room}} without knocking.\\ {\color{purple}Label}: \textbf{\texttt{Entity-Destination}}\\{\color{purple}Prediction w/o GIRL}: \textbf{\texttt{Other}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{Entity-Destination}}\end{tabular}                                                                 \\
\\
\begin{tabular}[c]{@{}l@{}}The {\color{red}\textit{disc}} in a disc {\color{blue}\textit{music box}} plays this function, with pins\\ perpendicular to the plane surface...\\
{\color{purple}Label}: \textbf{\texttt{Content-Container}}\\{\color{purple}Prediction w/o GIRL}: \textbf{\texttt{Component-Whole}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{Content-Container}}\end{tabular} \\
\\
\begin{tabular}[c]{@{}l@{}}{\color{red}\textit{Natural history}} {\color{blue}\textit{programmes}} began as live outside broadcasts\\ on BBC television in the early 1950s.\\ {\color{purple}Label}: \textbf{\texttt{Topic-Message
}}\\ {\color{purple}Prediction w/o GIRL}: \textbf{\texttt{Other}}\\ {\color{purple}Prediction w. GIRL}: \textbf{\texttt{Other}}\end{tabular}                                       \\ \thickhline
\end{tabular}
% \vspace{-0.1in}
\end{table}
